Domain Adaptable Prescriptive AI Agent for Enterprise

Despite advancements in causal inference and prescriptive AI, its adoption in enterprise settings remains hindered primarily due to its technical complexity. Many users lack the necessary knowledge and appropriate tools to effectively leverage these technologies. This work at the MIT-IBM Watson AI Lab focuses on developing the proof-of-concept agent, PrecAIse, a domain-adaptable conversational agent equipped with a suite of causal and prescriptive tools to help enterprise users make better business decisions. The objective is to make advanced, novel causal inference and prescriptive tools widely accessible through natural language interactions. The presented Natural Language User Interface (NLUI) enables users with limited expertise in machine learning and data science to harness prescriptive analytics in their decision-making processes without requiring intensive computing resources. We present an agent capable of function calling, maintaining faithful, interactive, and dynamic conversations, and supporting new domains.

==> acknowledgments.tex <==
%% acknowledgments.tex

% From mitthesis package
% Version: 1.01, 2023/10/16
% Documentation: https://ctan.org/pkg/mitthesis


\section*{Acknowledgments}
\addcontentsline{toc}{chapter}{Acknowledgments}
I would like to express my deepest appreciation to my mentor, Kristjan Greenewald, and my teammates, Wei Sun and Scott McFaddin, at IBM Research for their immense support at every stage of this project. Their trust and encouragement allowed me to advance my ideas confidently. I also extend my gratitude to other members at the MIT-IBM Watson AI Lab, including Onkar Bhardwaj, Veronique Demers, and Mikhail Yurochkin, for their valuable insights and advocacy. A special thanks to Priscilla Capistrano for her support and encouragement throughout the 6A graduate process. Finally, I am deeply grateful to my thesis advisor, Devavrat Shah, for his thorough reviews and guidance on my work.

==> biography.tex <==
%% biography.tex
%% This section is optional

% From mitthesis package
% Version: 1.01, 2023/10/16
% Documentation: https://ctan.org/pkg/mitthesis

% \chapter*{Biographical Sketch}
% \addcontentsline{toc}{chapter}{Biographical Sketch}

% <TODO: Fab was born on Mars on February 31st, 500BC under a blue moon...>

% Silas Whitcomb Holman was born in Harvard, Massachusetts on January 20, 1856. He received his S.B. degree in Physics from MIT in 1876, and then joined the MIT Department of Physics as an Assistant. He became Instructor in Physics in 1880, Assistant Professor in 1882, Associate Professor in 1885, and Full Professor in 1893. Throughout this period, he struggled with increasingly severe rheumatoid arthritis. At length, he was defeated, becoming Professor Emeritus in 1897 and dying on April 1, 1900.

% Holman's light burned brilliantly before his tragic and untimely death. He published extensively in thermal physics, and authored textbooks on precision measurement, fundamental mechanics, and other subjects. He established the original Heat Measurements Laboratory. Holman was a much admired teacher among both his students and his colleagues. The reports of his department and of the Institute itself refer to him frequently in the 1880's and 1890's, in tones that gradually shift from the greatest respect to the deepest sympathy.

% Holman was a student of Professor Edward C. Pickering, then head of the Physics department. Holman himself became second in command of Physics, under Professor Charles R. Cross, some years later. Among Holman's students, several went on to distinguish themselves, including: the astronomer George E. Hale ('90) who organized the Yerkes and Mt. Wilson observatories and who designed the 200 inch telescope on Mt. Palomar; Charles G. Abbot ('94), also an astrophysicist and later Secretary of the Smithsonian Institution; and George K. Burgess ('96), later Director of the Bureau of Standards. 

==> mydesign.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mydesign.tex}[2023/10/11 v1.03 Typographic design options for thesis]

%%%%%%%%%%  Color support  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Color package: xcolor. 
%% Change this if you prefer something else

\usepackage[hyperref,dvipsnames,svgnames,x11names]{xcolor}

%% can add option [table] to xcolor to use color in tables (see xcolor documentation)


%%%%%%%%%%  Hyperlink and line number colors  %%%%%%%%%%%%%%

\AtBeginDocument{
    % Using color names from xcolor package
    \hypersetup{
    	linkcolor=Blue3,
    	citecolor=Blue3,
    	urlcolor=violet,
    	filecolor=red, 
    %	anchorcolor=yellow,%  not all pdf viewers recognize this field (although Firefox does): hyperref issues a warning
    %	colorscheme=phelype,% overrides link, cite, url, file colors with a preset scheme, through \DocumentMetadata
    	}
    %
    \ifmit@lineno
	    \renewcommand{\linenumberfont}{\sffamily\mdseries\tiny\color{violet}}% line numbers will be sans-serif, medium weight, tiny, and violet
	\fi
}

%%%%%%%%%  Caption support  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% see documentation for details of how to customize captions

\RequirePackage{caption}
\RequirePackage{subcaption}


%%%%%%%%%  Customize list environments  %%%%%%%%%%%%%%%%%%%%
% 
% see documentation for details of how to customize lists

%\RequirePackage{enumitem}


%%%%%%%%%  Customize titles and section headings  %%%%%%%%%%
% 
% see documentation for details of how to customize headings

\RequirePackage{titlesec}

% these titlesec commands just automate the bold math in some headings (rest follows default styles)
\titleformat{\section}{\mathversion{bold}\normalfont\Large\bfseries}{\thesection }{1em}{}
\titleformat{\subsection}{\mathversion{bold}\normalfont\large\bfseries}{\thesubsection}{1em}{}
\titleformat{\subsubsection}{\mathversion{bold}\normalfont\normalsize\bfseries}{\thesubsubsection}{1em}{}

% ==> NOT every font includes a bold math version, so you may need to use other math macros in the headings to get bold math <==


%%%%%%%%%  Change page margins  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% The default thesis margin is 1 inch all around. You may want different margins (e.g., to add a gutter for binding),
% in which case you can use the \newgeometry command from the geometry package.  Refer to the package documentation
% for details.
%
% mitthesis defaults: [top=1in,bottom=1in,left=1in,right=1in,marginparwidth=50pt,headsep=12pt,footskip=0.5in]
%
% The following tells the geometry package to use a two-sided layout with a 1 cm binding offset on the inside 
% 	and 1 inch margins all around, reducing textwidth slightly (by 0.7 cm). See geometry documentation, Section 8.2.
%
%\newgeometry{twoside, bindingoffset=1cm,margin=1in,marginparwidth=50pt,headsep=12pt,footskip=0.5in}

